Tight Time-Space Lower Bounds for Constant-Pass Learning

In his breakthrough paper, Raz showed that any parity learning algorithm requires either quadratic memory or an exponential number of samples [FOCS'16, JACM'19]. A line of work that followed extended this result to a large class of learning problems. Until recently, all these results considered learning in the streaming model, where each sample is drawn independently, and the learner is allowed a single pass over the stream of samples. Garg, Raz, and Tal [CCC'19] considered a stronger model, allowing multiple passes over the stream. In the $2$-pass model, they showed that learning parities of size $n$ requires either a memory of size $n^{1.5}$ or at least $2^{\sqrt{n}}$ samples. (Their result also generalizes to other learning problems.) In this work, for any constant $q$, we prove tight memory-sample lower bounds for any parity learning algorithm that makes $q$ passes over the stream of samples. We show that such a learner requires either $\Omega(n^{2})$ memory size or at least $2^{\Omega(n)}$ samples. Beyond establishing a tight lower bound, this is the first non-trivial lower bound for $q$-pass learning for any $q\ge 3$. Similar to prior work, our results extend to any learning problem with many nearly-orthogonal concepts. We complement the lower bound with an upper bound, showing that parity learning with $q$ passes can be done efficiently with $O(n^2/\log q)$ memory.

==> parameters.tex <==

%Let $\epsilon$ be a sufficiently small constant.

Let $n = \log_2 |X|$ (dimension of unknowns), $n' = \log_2 |A|$ (dimension of samples). $T=2^{r}$ is the number of samples. About the learning matrix $M\in \{0,1\}^{A\times X}$: three parameters $k_{\ext},\ell_{\ext},r_{\ext}$.

\begin{itemize}
    \item $\ell_{\ext}$: As soon as $\|\doubleP_{x|v}\|_2\le 2^{-n} \cdot 2^{\ell_{\ext}}$, one can apply the extractor property of $M$.
    \item $k_{\ext}$: when one applies the extractor property of $M$, at most $2^{-k_{\ext}}$-fraction of all examples $a\in A$ are ``bad''.
    \item $r_{\ext}$: for every non-bad example $a\in A$, it holds that 
    \[
    \Pr_{x\sim \doubleP_{x|v}}[M(a,x)=0] \in \left( \frac{1}{2} - 2^{-r_{\ext}}, \frac{1}{2} + 2^{-r_{\ext}}\right).
    \]
\end{itemize}

For all passes, the following parameters apply.

\begin{itemize}
    \item $T = 2^\rlen$ is the number of samples (equivalently the length of one pass). We assume that $\rlen \le \frac{\ell}{3}$.
    \item $\ellsigv$: the threshold for significant values, \emph{across all passes}. We assume $\ellsigv \ge 100^{q}\cdot \ell$ where $q$ is the number of passes.
    \item Memory lower bound we wish to prove: $2^{\frac{1}{16}k\ell}$.
    \item Stopping probability upper bound we wish to derive $2^{-\rlen+O(1)}$.
\end{itemize}

For the first pass:
\begin{itemize}
    \item Threshold for significant states is $2^{\ell^{(1)}_s}\cdot 2^{-n}$ where $\ell^{(1)}_s = \ell$.
    \item Threshold for flat distribution is $2^{\ell^{(1)}_f}\cdot 2^{-n}$ where $\ell^{(1)}_f = 2\ell^{(1)}+2\rlen$.
\end{itemize}

For the second pass,
\begin{itemize}
\item The threshold for high-probability edges is $L_{\high} = \ell$.
\item The threshold for the counter is $L_{\cnt} = L_{\high} + 7\ell$.
\item The state threshold is $2^{\ell^{(2)}_s}\cdot 2^{-n}$ where $\ell^{(2)}_s = 10\ell$.
\item The value threshold is $2^{\ell^{(2)}_v} \cdot 2^{-n}$ where $\ell^{(2)}_v = 22\ell$.
\end{itemize}



% About the branching program parameters,

% % \begin{itemize}
% %     \item mm: The length of BP in one pass. In original two pass, m = 2^{\epsilon \cdot \min(r, k, \sqrt{l})m = 2^{\epsilon \cdot \min(r, k, \sqrt{l})
% %     \item dd: The width of BP. Not important, only used in the union bound. In original two pass, d = 2^{\epsilon k \cdot \min(k, \sqrt{l})d = 2^{\epsilon k \cdot \min(k, \sqrt{l})
% % \end{itemize}

% About the stopping rules in the first pass,

% \begin{itemize}
%     \item $l^{(1)}$: Significant vertex stop rule. $||P_{x|v_0 \to v}||_2 > 2^{-n + l^{(1)}}$.
%     \item $l_{sigv}^{(1)}$: Significant value stop rule. $P_{x|v_0 \to v}(x') > 2^{-n+l_{sigv}^{(1)}}$.
%     \item $r_{bad}^{(1)}$: Bad edge stop rule. $\Pr_{x\sim \doubleP_{x|v_0\to v}}[M(a,x)=1] \not\in \left( \frac{1}{2}-2^{-r_{bad}^{(1)}},\frac{1}{2}+2^{-r_{bad}^{(1)}} \right)$
% \end{itemize}

% About the stopping rules in the second pass,

% \begin{itemize}
%     \item $l^{(2)}$: Significant vertex stop rule. $||P_{x|v_1 \to v}||_2 > 2^{-n + l^{(2)}}$.
%     \item $l_{sigv}^{(2)}$: Significant value stop rule. $P_{x|v_1 \to v}(x') > 2^{-n+l_{sigv}^{(2)}}$.
%     \item $r_{bad}^{(2)}$: Bad edge. $\Pr_{x\sim \doubleP_{x|v_1\to v}}[M(a,x)=1] \not\in \left( \frac{1}{2}-2^{-r_{bad}^{(2)}},\frac{1}{2}+2^{-r_{bad}^{(2)}} \right)$
%     \item $k_{high}^{(2)}$: High probability edge. $\Pr[a_{i+1}=a|v_0 \wt v] \ge 2^{-k_{high}^{(2)}}$ 
% \end{itemize}

\subsection*{Parameter inequalities}


